From High-Level Modeling Towards Efficient and Trustworthy Circuits

Behavior-Interaction-Priority (BIP) is a layered embedded system design and verification framework that provides separation of functionality, synchronization, and priority concerns to simplify system design and to establish correctness by construction. The framework comes with a runtime engine and a suite of verification tools that uses D-Finder and NuSMV as model checkers. In this paper we provide a method and a supporting tool that takes a BIP system and a set of invariants and computes a reduced sequential circuit with a system-specific scheduler and with a designated output that is true when the invariants hold. Our method uses ABC, a sequential circuit synthesis and verification framework to (1) generate an efficient FPGA implementation of the system, and to (2) verify the system and debug it in case a counterexample was found. Moreover we generate a concurrent C implementation of the circuit that can be directly used as a simulator. We evaluated our method with two large systems and our results outperform those possible with existing techniques.

==> translation-tmp.tex <==
\section{Translation from BIP to Sequential Circuit}
\label{sect-translation}



\begin{lstlisting}
decl-list

wiredef-list

do_together {
  init-list
}

while(true) {
  do_together {
    next-list
  }
}
\end{lstlisting}

\begin{lstlisting}
($\pi\big(\gamma(\{B_i\}_{i \in I})\big)$, K), where $\gamma = \{a_j\}_{j \in J}$

/***************** declarations ******************/
// interaction wires
decl-list += wire bool ie[|J|]; // interaction enablement 
decl-list += wire bool ip[|J|]; // interaction priority
decl-list += wire bool is[|J|]; // interaction selected

decl-list += wire int selector; // non-deterministic priority selector

decl-list += bool cycle; // cycle denotes whether we are executing an interaction or a transition 

foreach $i \in [1..|I|]$

  foreach $j \in [1..|B_i.P|]$ // where $B_i.P = \{p_1, \ldots, p_{|B_i.P|}\}$ 
    decl-list += wire bool $B_i.p_j.e$; // port enablement
    decl-list += wire bool $B_i.p_j.s$; // port selected
  endfor 
  
  decl-list += int $B_i.\ell$;
  
  foreach $j \in [1..|B_i.X|]$ // where $B_i.X = \{x_1, \ldots, x_{|B_i.X|}\}$  
    decl-list += int $B_i.x_j$; // variable registers
  endfor
   
endfor
\end{lstlisting}

\iffalse
\begin{lstlisting}
  BIP2$\this$($\pi\big(\gamma(\{B_1, \ldots, B_n\})\big)$, K)
  Let bW, bR, bPI be the set of Boolean wire, register and primary input variables, respectively.
  Let W, R, PI be the set of integer wire, register and primary input variables, respectively.
  Let wiredef, init, next be empty lists of statements. 

  foreach component $B \in \{B_1, \ldots, B_n\}$
    R += $B_i\_{\ell}$ // location register variable
    foreach variable $x$ in $B_i.X$
      R +=  $B_i$_x
    foreach port $p$ in $B_i.P$ 
      bW += $\{ B_i\_p\_\mathit{enable}, B_i\_p\_\mathit{selected}\}$

  foreach interaction  $a_i \in \gamma$
    $a\_enable[i] = G_{a_i} \wedge \bigwedge_{p\in P_{a_i}\wedge p=B_i.p } B_i.p\_selected  $ 
    $a\_execute[i] = $
    $a\_piority[i] = $
\end{lstlisting}
\fi

\begin{lstlisting}
/***************** wire list definitions ******************/
foreach $j \in [1..|J|]$
  wiredef-list += ie[j] := $a_j.guard \wedge \bigwedge_{p\in a_i.P} component(p).p.e$ 
  wiredef-list += ip[j] := ie[j] $\wedge \,(\forall k \neq j: ie[k] \Rightarrow a_k < a_j)$ 
  wiredef-list += is[j] := ip[j] $\wedge \,(selector = j \vee \forall k > j: \neg ip[k])$   
endfor


foreach $i \in [1..|I|]$

  foreach $j \in [1..|B_i.P|]$ // where $B_i.P = \{p_1, \ldots, p_{|B_i.P|}\}$ 
    wiredef-list += $B_i.p_j.e := \bigvee_{\tau \in transitions(B_i.p)} \tau.guard$; 
    wiredef-list += $B_i.p_j.s := \bigvee_{a_k \in interactions(B_i.p_j)} a_k$; 
  endfor 
endfor
\end{lstlisting}
\todo[inline=true]{
define interactions(port), component(port), transitions(port)
}

\begin{lstlisting}
/***************** init list definitions ******************/
init-list += $cycle := 0$; // where dot is the relational product

foreach $i \in [1..|I|]$
  init-list += $B_i.\ell := Init.B_i$; // where dot is the relational product
  foreach $j \in [1..|B_i.X|]$ // where $B_i.X = \{x_1, \ldots, l_{|B_i.X|}\}$ 
    init-list += $B_i.x_j := v(B_i.x_j)$; // v is the initial valuation
  endfor 
endfor
\end{lstlisting}


\begin{lstlisting}
/***************** next list definitions ******************/
foreach $i \in [1..|I|]$
  foreach $j \in [1..|B_i.X|]$ // where $B_i.X = \{x_1, \ldots, l_{|B_i.X|}\}$ 
    st = $B_i.x_j$ := cycle = 0?
    foreach $k \in [1..|J|]$
      foreach assignment $\sigma \in a_k.action$
        if($B_i.x_j = \sigma.term$)
          $st += is[k]?\, \sigma.expr:$
        endif
      endfor
    endfor
    
    st += B_i.x_j:  
    foreach $\tau \in B_i.T$ 
      foreach assignment $\sigma \in \tau.action$
        if($B_i.x_j = \sigma.term$)
          $st += B_i.port(\tau).s?\, \sigma.expr:$
        endif
      endfor
    endfor      
    $st += B_i.x_j$; 
    next-list += st;  
  endfor
  $next-list += cycle := \neg cycle$; 
endfor
\end{lstlisting}

This section presents how we translate a BIP system $(B,\mathit{Init}, v)$ to its corresponding sequential circuit  $\big( (V, E),G, O\big)$. 



